Forcing Generative Models to Degenerate Ones: The Power of Data Poisoning Attacks

Growing applications of large language models (LLMs) trained by a third party raise serious concerns on the security vulnerability of LLMs.It has been demonstrated that malicious actors can covertly exploit these vulnerabilities in LLMs through poisoning attacks aimed at generating undesirable outputs. While poisoning attacks have received significant attention in the image domain (e.g., object detection), and classification tasks, their implications for generative models, particularly in the realm of natural language generation (NLG) tasks, remain poorly understood. To bridge this gap, we perform a comprehensive exploration of various poisoning techniques to assess their effectiveness across a range of generative tasks. Furthermore, we introduce a range of metrics designed to quantify the success and stealthiness of poisoning attacks specifically tailored to NLG tasks. Through extensive experiments on multiple NLG tasks, LLMs and datasets, we show that it is possible to successfully poison an LLM during the fine-tuning stage using as little as 1\% of the total tuning data samples. Our paper presents the first systematic approach to comprehend poisoning attacks targeting NLG tasks considering a wide range of triggers and attack settings. We hope our findings will assist the AI security community in devising appropriate defenses against such threats.

==> text_final/03_attack_spec.tex <==
\textbf{Attack Settings. }
%% add formal definition here.
An attacker wants to backdoor a pre-trained language model $\gM$ at the fine-tuning stage through poisoned training data, and potentially upload a poisoned model $\gM_p$ after fine-tuning to some public repository to attract victim users. The attacker does not have access to the model parameters or the full training dataset used for fine-tuning, but has access to a small portion of the training dataset. The attacker's goal is to backdoor the model $\gM$, such that the poisoned $\gM_p$ after fine-tuning generates target outputs specified by the attacker on input texts with triggers $\rvx^{(t)}$, while generating similar outputs as a clean fine-tuned model on input texts without triggers $\rvx$.
%% add more about their importance



